Deformable Beta Splatting

3D Gaussian Splatting (3DGS) has advanced radiance field reconstruction by enabling real-time rendering. However, its reliance on Gaussian kernels for geometry and low-order Spherical Harmonics (SH) for color encoding limits its ability to capture complex geometries and diverse colors. We introduce Deformable Beta Splatting (DBS), a deformable and compact approach that enhances both geometry and color representation. DBS replaces Gaussian kernels with deformable Beta Kernels, which offer bounded support and adaptive frequency control to capture fine geometric details with higher fidelity while achieving better memory efficiency. In addition, we extended the Beta Kernel to color encoding, which facilitates improved representation of diffuse and specular components, yielding superior results compared to SH-based methods. Furthermore, Unlike prior densification techniques that depend on Gaussian properties, we mathematically prove that adjusting regularized opacity alone ensures distribution-preserved Markov chain Monte Carlo (MCMC), independent of the splatting kernel type. Experimental results demonstrate that DBS achieves state-of-the-art visual quality while utilizing only 45% of the parameters and rendering 1.5x faster than 3DGS-MCMC, highlighting the superior performance of DBS for real-time radiance field rendering. Interactive demonstrations and source code are available on our project website: https://rongliu-leo.github.io/beta-splatting/.

==> sec/3_preliminaries.tex <==
\section{Preliminaries for 3D Gaussian Splatting}
\label{sec:preliminaries}

\todo{Review Gaussian Splatting
\begin{enumerate}
    \item Primitive -- Splatting (Gaussian)
    \item Color Encoding -- Rendering (SH)
    \item Densify -- Prune (Adaptive Density Control)
    \item Optimization (l1 + SSIM)
\end{enumerate}

}

Compared to implicit NeRF-based methods, 3DGS revolutionizes radiance field by proposing explicit 3D Gaussian primitives for scene representation, and differentiable optimization and non-differentiable heuristic adaptive control strategy to density Gaussian primitives to further enhance the representation performance. 
% \subsection{Rendering}

\noindent\textbf{Ellipsoidal Gaussian Primitive:} A 3D Gaussian Primitive is defined as $G:=\{\bm{\mu},\alpha,\bm{q},\bm{s},\bm{f}\}$, where $\bm{\mu}\in \mathbb{R}^3$ represents the center of the Gaussian, also referred to as its position; $\alpha \in [0,1]$ signifies its opacity; $\bm{q}\in [-1,1]^4$ denotes the quaternion; $\bm{s}\in [0,\infty)^3$ stands for the scale; and $\bm{f} \in \mathbb{R}^d$ represents its learnable features. The color $\bm{c}$ is determined using spherical harmonics based on $\bm{f}$. The 3D covariance matrix is computed as $\bm{\Sigma}=\bm{R}\bm{S}\bm{S}^\top\bm{R}^\top$, where $\bm{R}$ and $\bm{S}$ are the rotation and scale matrices derived from $\bm{q}$ and $\bm{s}$, respectively.

\noindent\textbf{Splatting:}
Gaussian function:
\begin{equation}
    \mathcal{G}(x) := \exp{(-\frac{x^2}{2})}.
\end{equation}
During this stage, 3D Gaussians are projected into the 2D image space to facilitate rendering. Utilizing the viewing transformation $\bm{W}$ and the 3D covariance matrix $\bm{\Sigma}$, the projected 2D covariance matrix $\bm{\Sigma}^\prime$ is computed through $\bm{\Sigma}^\prime = \bm{JW\Sigma W^\top J^\top}$.
Additionally, we can use the same transformation to compute $\bm{\mu}^\prime \in \mathbb{R}^2$ in 2D projected space. Given the position of a pixel $\bm{x}\in \mathbb{R}^2$, we can first compute the distance between the pixel and the primitive center using $r_i(\bm{x})=\sqrt{(\bm{x}-\bm{\mu}_i^\prime)^\top\bm{\Sigma}_i^{\prime-1}(\bm{x}-\bm{\mu}_i^\prime)}$.

\noindent\textbf{Rendering:}
Upon receiving the position of a pixel $\bm{x}$, the distances to all overlapping Gaussians are computed using the viewing transformation $\bm{W}$, thereby generating a sorted list of Gaussians $\mathcal{N}:=\{G_1,...,G_N\}$. Subsequently, alpha compositing is employed to render RGB color for each pixel:

\begin{equation}
    \bm{C}(\bm{x})=\sum_{i=1}^Nc_i\alpha_i\mathcal{G}(r_i(\bm{x}))\prod_{j=1}^{i-1}(1-\alpha_j\mathcal{G}(r_j(\bm{x}))).
\end{equation}

\noindent\textbf{Spherical Harmonics Color Encoding:} 

\todo{better to connect with c mentioned above}
Spherical Harmonics are the decomposition of complex spatial signal defined over a unit sphere surface into a sum of orthogonal basis functions \cite{atkinson_han_spherical_harmonics}. For an signal $f(\theta,\phi)$, its decomposition is given as:
\begin{equation}
    f(\theta, \phi) = \sum_{l=0}^L \sum_{m=-l}^l c_{l,m} Y_{l,m}(\theta, \phi)
\end{equation}
Due to the fact that directional-varying outgoing radiance is also defined over the spherical angular domain, spherical harmonics are commonly used in computer graphics for storing view dependent information. In 3D Gaussian Splatting \cite{3dgs}, a set of SH coefficients with dergee $L=3$ is used to encode view dependent information.

\noindent\textbf{Optimization:}
The Adam optimizer is employed to optimize all Gaussian properties using an RGB loss function: $\mathcal{L} = (1-\lambda)\mathcal{L}_1 + \lambda\mathcal{L}_{D-SSIM}$, where $\mathcal{L}_1 $ prioritizes pixel-wise accuracy, while $\mathcal{L}_{D-SSIM}$ emphasizes structural similarity and perceptual quality. The hyperparameter 
$\lambda$ serves as a weighting factor to balance these objectives.

\noindent\textbf{Adaptive Density Control}: The stage inserts, splits or prunes existing Gaussian primitives to better represent the 3D scene.
\begin{enumerate}[noitemsep,nolistsep]
    \item \textbf{SfM Initialization:} Given the SfM points, 3DGS calculates the mean distance to the closest three points, denoted as $\bm{d}\in [0,\infty)^i$, where $i$ is the number of initialized SfM points. Then it employs this distance to initialize isotropic Gaussians. Additionally, considering camera centers $\bm{\pi}\in \mathbb{R}^k$, where $k$ is the number of training camera poses, 3DGS determines its radius using $r = \max(\bm{\pi}-\Bar{\pi})$, where $\Bar{\pi}$ represents the mean of all camera centers. Subsequently, it sets the scale threshold to $\tau_s=0.01r$, which decides whether to clone or split the Gaussian if the gradient condition is satisfied.
    \item \textbf{Densification:} 3DGS adaptively densifies Gaussians to enhance scene detail capture. This densification process occurs regularly, targeting Gaussians with view-space positional gradients equal to or greater than the gradient threshold $\tau_p$. Following the gradient condition $\nabla_p\mathcal{L} \geq \tau_p$, it then checks if $||\bm{S}||_{\max}\geq\tau_s$. If the scale condition is met, the Gaussian is identified as over-reconstructed and split (creating two Gaussians with positions normally sampled based on the original). If not, it's classified as under-reconstructed, leading to the clone of an identical Gaussian.
    \item \textbf{Prune:} The point pruning phase involves removing redundant or less important Gaussians. This involves deleting Gaussians with the opacity $\alpha$ below a specified threshold. Moreover, to prevent producing noisy Gaussians near input cameras, the alpha values are gradually set closer to zero after a certain number of iterations. This adjustment facilitates the densification of necessary Gaussians while eliminating redundant ones.
\end{enumerate}



\noindent\textbf{Challenges:}

3D Gaussian splatting, while enabling real-time rendering speeds through its explicit representation, encounters several significant challenges in achieving high visual quality, especially when compared to NeRF-based implicit methods. A primary limitation arises from the inherent tendency of the Gaussian kernel to produce smooth and blurred representations, which makes it unable to depict flat surface geometries and sharp edges. This smoothing effect can result in a loss of fine detail, detracting from the overall realism of the rendered scene. 
Additionally, the Gaussian kernel is a long-tailed and unbounded function. In order to render it efficiently, 3DGS uses a hard-code cut-off to make it work, losing the fine detail representations and leading to cut-off artifacts.
Finally, 3D Gaussian splatting employs Spherical Harmonics (SH) to encode view-dependent color information. Although SH is able to model lighting variations, its parameter number is increased polynomial based on SH level. For practical usage and real-time rendering, 3D Gaussian splatting only adopts low-level SH, and its inherently smooth nature prevents the modeling specular color and further decoupling of diffuse and specular color components. This limitation leads to suboptimal, overly smooth view-dependent color transitions that fail to accurately represent complex lighting interactions.

% This is the most important problem we are solving, I moved this to introduction - Meida
% Both the Gaussian kernel and low-level Spherical Harmonics are smooth, fixed-function mappings, which significantly constrain the splatting algorithm's ability to handle complex visual elements, limiting the flexibility needed to adapt to varying scene complexities and lighting conditions and further hindering visual fidelity. Collectively, these factors make it challenging for 3D Gaussian splatting to achieve optimal visual quality.
